Locating the intense interstellar scattering towards the inner Galaxy

We use VLBA+VLA observations to measure the sizes of the scatter-broadened images of 6 of the most heavily scattered known pulsars: 3 within the Galactic Centre (GC) and 3 elsewhere in the inner Galactic plane. By combining the measured sizes with temporal pulse broadening data from the literature and using the thin-screen approximation, we locate the scattering medium along the line of sight to these 6 pulsars. At least two scattering screens are needed to explain the observations of the GC sample. We show that the screen inferred by previous observations of SGR J1745-2900 and Sgr A*, which must be located far from the GC, falls off in strength on scales < 0.2 degree. A second scattering component closer to (< 2 kpc) or even (tentatively) within (< 700 pc) the GC produces most or all of the temporal broadening observed in the other GC pulsars. Outside the GC, the scattering locations for all three pulsars are ~2 kpc from Earth, consistent with the distance of the Carina-Sagittarius or Scutum spiral arm. For each object the 3D scattering origin coincides with a known HII region (and in one case also a supernova remnant), suggesting that such objects preferentially cause the intense interstellar scattering seen towards the Galactic plane. We show that the HII regions should contribute > 25% of the total dispersion measure (DM) towards these pulsars, and calculate reduced DM distances. Those distances for other pulsars lying behind HII regions may be similarly overestimated.

==> vlbavla_size_table.tex <==
%\documentclass{article}
%\begin{document}
%\footnotesize
\begin{table*}
\caption{\label{sizetable}Sizes and positions for detected sources.}
\begin{tabular}{lcllcl}
\hline
 Source      &   Obs. freq. (GHz) & RA & DEC & FWHM size (mas) & $1 \sigma$ range\\
\hline
 J1745$-$2912 &  8.7  &      17:45:47.83043(23) &  -29:12:30.780(3) & 
      1.7 & [0.3, 3.1]      \\
 J1746$-$2849  & 8.7 &        17:46:03.35736(12) &  -28:50:13.385(2) &       5.3 & [2.6, 8.0]      \\
 J1746$-$2856  &  5.9 &      17:46:49.85480(6) &  -28:56:58.990(1) &     10.9   & [9.7, 12.1]  \\
 B1758$-$23    &  7.5  &      18:01:19.81488(60) &  -23:04:44.637(10) & 
     12.5 & [10.3, 14.5]     \\
 B1809$-$176   &  4.5 &        18:12:15.85925(17) & -17:33:37.871(2) &  
    17.6 & [10.3, 24.7]      \\
 B1822$-$14    &  7.5   &    18:25:02.95832(1) & -14:46:53.3605(2) &1.8 & [1.7, 2.0]      \\
\hline


\end{tabular}
\end{table*}
